Detection and Evaluation of bias-inducing Features in Machine learning

The cause-to-effect analysis can help us decompose all the likely causes of a problem, such as an undesirable business situation or unintended harm to the individual(s). This implies that we can identify how the problems are inherited, rank the causes to help prioritize fixes, simplify a complex problem and visualize them. In the context of machine learning (ML), one can use cause-to-effect analysis to understand the reason for the biased behavior of the system. For example, we can examine the root causes of biases by checking each feature for a potential cause of bias in the model. To approach this, one can apply small changes to a given feature or a pair of features in the data, following some guidelines and observing how it impacts the decision made by the model (i.e., model prediction). Therefore, we can use cause-to-effect analysis to identify the potential bias-inducing features, even when these features are originally are unknown. This is important since most current methods require a pre-identification of sensitive features for bias assessment and can actually miss other relevant bias-inducing features, which is why systematic identification of such features is necessary. Moreover, it often occurs that to achieve an equitable outcome, one has to take into account sensitive features in the model decision. Therefore, it should be up to the domain experts to decide based on their knowledge of the context of a decision whether bias induced by specific features is acceptable or not. In this study, we propose an approach for systematically identifying all bias-inducing features of a model to help support the decision-making of domain experts. We evaluated our technique using four well-known datasets to showcase how our contribution can help spearhead the standard procedure when developing, testing, maintaining, and deploying fair/equitable machine learning systems.

==> double-swap-function.tex <==
%\subsection{Algorithm}

%% https://shantoroy.com/latex/how-to-write-algorithm-in-latex/
\begin{algorithm}[!ht]
\caption{Double Features Swapping function (Case 1)}
\label{algo:double-swap-swap}
\DontPrintSemicolon
  
  \KwInput{$x^f, x^m, r, d^*$} %\tcp*{r and d are optionall}
  \KwData{Testing set $X$}
  \KwRequired{Temporal ordering: $x^f\to x^m$}
  \KwOutput{$X', X''$}
  %$\sum_{i=1}^{\infty} := 0$ \tcp*{this is a comment}
  \tcc{Start by getting the total length of the input data}
  $N \gets length(X)$
  
  %$\text{SwapColumnIndex } \gets \text{getColumnIndexOf}(x^f)$
  
  %$\text{MediatorColumnIndex } \gets \text{getColumnIndexOf}(x^m)$
  
  $\text{RandomIndex } \gets$ 
  $\text{getRandomIndex}(\text{range}(0,N))$
  
  \tcc{Swap feature value categories}
  $fC_1 \gets \text{getFirstBinValuesOf}(x^f)$
  
  $fC_2 \gets \text{getSecondBinValuesOf}(x^f)$
  
  \tcc{Mediator values categories}
  $mC_1 \gets \text{getFirstBinValuesOf}(x^m)$
  
  $mC_2 \gets \text{getSecondBinValuesOf}(x^m)$
  
  $X' = \text{createEmptyList}()$\tcp*{Create empty list to store the first tuple}
  
  $X'' = \text{createEmptyList}()$ \tcp*{Create empty list to store the second tuple}
  
  $\text{distortedIndices} = \text{createEmptyList}()$
  
  \For{$cm \gets [c_1, c_2]$}
  {
      \For{$i \gets range(0, N)$}
      {
      \If{$i$ in $getRandomIndex$}
      {
       $x_i$ = getDataPointAt($i$)
       
       %$Xi_{value}^f$ = getRandomValue($x_i$, $\text{getColumnIndexOf}(x^f)$)
       
       \If{$Xi_{value}^f == c_m$}
       {
            %$x_i$ = getDataPointAt($i$)
            \tcc{Interchange the mediator value}
            %$Xi_{value}^m$ = getRandomValue($x_i$, MediatorColumnIndex)
            \tcc{When performing swapping, the current value of $x^m$ in row $x_i$ is compared with the categories $mC1$ or $mC2$, and the random value from the alternative category is chosen and replaced with the current value of $x^m$ in $x_i$}
            $x_i'$ = SwitchValueof($x_i$, AtIndexof($x^m$))
       
            %\If{$Xi_{value}^m \text{ in } mC_1$}
           % {
           %     $RandomC_{2}$ = chooseRandomValueFrom($mC_2$)
                 
           %      $x_i'$ = setValuef($x_i$,MediatorColumnIndex) = $RandomC_{2}$ 
           % } 
           %\Else
           % {
           %   $RandomC_{1}$ = chooseRandomValueFrom($mC_1$)
              
            %  $x_i' = \text{setValue}(x_i,\text{MediatorColumnIndex}) \text{ to } RandomC_{1}$
          % }
          \tcc{Make a copy of the swapped data point before swapping the feature value}
           $x_i''$ = copy($x_i'$)
           
           \tcc{Interchange the PBF value}
           \tcc{During the swapping the current value of $x^f$ is compared with the category $fC1$ or $fC2$, and the random value from the alternative category is chosen and replaced with the current value of $x^f$ in $x_i'$}
           $x_i''$ = SwitchValueof($x_i'$, AtIndexof($x^f$))
            %\If{$Xi_{value}^f \text{ in } fC_1$}
            %{
            %    $RandomC_{2}$ = chooseRandomValueFrom($fC_2$)
                 
            %     $x_i''$ = setValuef($x_i'$,$\text{getColumnIndexOf}(x^f)$) = $RandomC_{2}$ 
            %} 
           %\Else
            %{
            %      $RandomC_{1}$ = chooseRandomValueFrom($fC_1$)
                  
            %      $x_i'' = \text{setValue}(x_i',\text{SwapColumnIndex}) \text{ to } RandomC_{1}$
            %}
            
       }
       \tcc{The distortion of the first and second post-swapped data $x'$, $x''$ is compared with $\bm{d^*}$}
       
       distortion = \text{measureStatisticalDistanceBetween}$(x_i', x_i'')$
       
       \If{$distortion \leq \bm{d^*}$}{
          $X'$.append$(x_i')$ \tcp*{save the swapped data}
          $X''$.append$(x_i'')$ \tcp*{save the swapped data}
          
          \tcc{Save the indices of the swapped data-points.}
        
        $\text{distortedIndices}$.append$(i)$ 
       }
       %\Else
       %{
       % $X'$.append$(x_i)$ \tcp*{save the original data}
       %}
      }
      %\Else
      %{
      %$X'$.append$(x_i)$ \tcp*{save the original data as it is}
      %}
      }
  }
  \Return{$X', X''$}
  %\If{Condition 1}
  %  {
  %      Do something    \tcp*{this is another comment}
  %      \If{sub-Condition}
  %      {Do a lot}
  %  }
  %  \ElseIf{Condition 2}
  %  {
  %  	Do Otherwise \;
  %      \tcc{Now this is a for loop}
  %      \For{sequence}    
  %      { 
  %      	loop instructions
  %      }
  %  }
  %  \Else
  %  {
  %  	Do the rest
  %  }
    
  %  \tcc{Now this is a While loop}
  % \While{Condition}
  % {
  % 		Do something\;
  % }
\end{algorithm}

==> double-swap-function2.tex <==
%\subsection{Algorithm}

%% https://shantoroy.com/latex/how-to-write-algorithm-in-latex/
\begin{algorithm}[!ht]
\caption{Double Features Swapping function (Case 2)}
\label{algo:double-swap-swap}
\DontPrintSemicolon
  
  \KwInput{$x^f, x^m, r, d^*$} %\tcp*{r and d are optionall}
  \KwData{Testing set $X$}
  \KwRequired{Temporal priority ordering: $x^f\to x^m$}
  \KwOutput{$X', X''$}
  %$\sum_{i=1}^{\infty} := 0$ \tcp*{this is a comment}
  \tcc{Start by getting the total length of the input data}
  $N \gets length(X)$
  
  %$\text{SwapColumnIndex } \gets \text{getColumnIndexOf}(x^f)$
  
  %$\text{MediatorColumnIndex } \gets \text{getColumnIndexOf}(x^m)$
  
  $\text{RandomIndex } \gets$ 
  $\text{getRandomIndex}(\text{range}(0,N))$
  
  \tcc{Swap feature value categories}
  $fC_1 \gets \text{getFirstBinValuesOf}(x^f)$
  
  $fC_2 \gets \text{getSecondBinValuesOf}(x^f)$
  
  \tcc{Mediator values categories}
  $mC_1 \gets \text{getFirstBinValuesOf}(x^m)$
  
  $mC_2 \gets \text{getSecondBinValuesOf}(x^m)$
  
  $X' = \text{createEmptyList}()$\tcp*{Create empty list to store the first tuple}
  
  $X'' = \text{createEmptyList}()$ \tcp*{Create empty list to store the second tuple}
  
  $\text{distortedIndices} = \text{createEmptyList}()$
  
  \For{$cm \gets [c_1, c_2]$}
  {
      \For{$i \gets range(0, N)$}
      {
      \If{$i$ in $getRandomIndex$}
      {
       $x_i$ = getDataPointAt($i$)
       
       %$Xi_{value}^f$ = getRandomValue($x_i$, $\text{getColumnIndexOf}(x^f)$)
       
       \If{$Xi_{value}^f == c_m$}
       {
            %$x_i$ = getDataPointAt($i$)
             \tcc{Interchange the PBF value}
           \tcc{During the swapping the current value of $x^f$ is compared with the category $fC1$ or $fC2$, and the random value from the alternative category is chosen and replaced with the current value of $x^f$ in $x_i$}
           $x_i'$ = SwitchValueof($x_i$, AtIndexof($x^f$))
           
            %\If{$Xi_{value}^m \text{ in } mC_1$}
           % {
           %     $RandomC_{2}$ = chooseRandomValueFrom($mC_2$)
                 
           %      $x_i'$ = setValuef($x_i$,MediatorColumnIndex) = $RandomC_{2}$ 
           % } 
           %\Else
           % {
           %   $RandomC_{1}$ = chooseRandomValueFrom($mC_1$)
              
            %  $x_i' = \text{setValue}(x_i,\text{MediatorColumnIndex}) \text{ to } RandomC_{1}$
          % }
          \tcc{Make a copy of the swapped data point before swapping the mediator values}
           $x_i''$ = copy($x_i'$)
           
           \tcc{Interchange the mediator value}
            %$Xi_{value}^m$ = getRandomValue($x_i$, MediatorColumnIndex)
            \tcc{When performing swapping, the current value of $x^m$ in row $x_i'$ is compared with the categories $mC1$ or $mC2$, and the random value from the alternative category is chosen and replaced with the current value of $x^m$ in $x_i'$}
            $x_i''$ = SwitchValueof($x_i'$, AtIndexof($x^m$))
          
            %\If{$Xi_{value}^f \text{ in } fC_1$}
            %{
            %    $RandomC_{2}$ = chooseRandomValueFrom($fC_2$)
                 
            %     $x_i''$ = setValuef($x_i'$,$\text{getColumnIndexOf}(x^f)$) = $RandomC_{2}$ 
            %} 
           %\Else
            %{
            %      $RandomC_{1}$ = chooseRandomValueFrom($fC_1$)
                  
            %      $x_i'' = \text{setValue}(x_i',\text{SwapColumnIndex}) \text{ to } RandomC_{1}$
            %}
            
       }
       \tcc{Compare the distortion of post-swapped  and pre-swapped data with $d^*$}
       
       distortion = \text{measureStatisticalDistanceBetween}$(x_i', x_i'')$
       
       \If{$distortion \leq d^*$}{
          $X'$.append$(x_i')$ \tcp*{save the swapped data}
          $X''$.append$(x_i'')$ \tcp*{save the swapped data}
          
          \tcc{Save the indices of the swapped data-points.}
        
        $\text{distortedIndices}$.append$(i)$ 
       }
       %\Else
       %{
       % $X'$.append$(x_i)$ \tcp*{save the original data}
       %}
      }
      %\Else
      %{
      %$X'$.append$(x_i)$ \tcp*{save the original data as it is}
      %}
      }
  }
  \Return{$X', X''$}
  %\If{Condition 1}
  %  {
  %      Do something    \tcp*{this is another comment}
  %      \If{sub-Condition}
  %      {Do a lot}
  %  }
  %  \ElseIf{Condition 2}
  %  {
  %  	Do Otherwise \;
  %      \tcc{Now this is a for loop}
  %      \For{sequence}    
  %      { 
  %      	loop instructions
  %      }
  %  }
  %  \Else
  %  {
  %  	Do the rest
  %  }
    
  %  \tcc{Now this is a While loop}
  % \While{Condition}
  % {
  % 		Do something\;
  % }
\end{algorithm}
